Interaction dynamics in 'Friends'

Computational narrative analysis increasingly seeks representations that capture how language reflects changing social and interactional contexts. We apply Ousiometry, a lexicon-based framework organized around Power, Danger, and Structure, to the complete dialogue of Friends (236 episodes, 750K tokens), examining temporal variation, group-level positioning, and pairwise co-variation among the six main characters. We find substantial episode-to-episode fluctuation in character trajectories, with PELT-detected change points descriptively aligning with major narrative events. At the group level, character combinations occupy different regions of Power--Danger space, with greater dispersion in Power than Danger, although these differences do not survive Bonferroni correction and trajectory clustering shows weak structure (silhouette = 0.27). Pairwise Pearson correlations reveal modest co-variation across characters, with three significant pairs in Power, two in Danger, and six in Structure after correction. Partial correlations substantially reduce these associations, leaving only one significant pair in Power and one in Danger, suggesting that much of the observed co-variation reflects ensemble-wide rather than pair-specific dynamics. Overall, our findings show that episode-level Ousiometry captures meaningful temporal variation in character dialogue, while evidence for stable group-level structure and pair-specific co-variation remains limited. Semantic variation in Friends is therefore better characterized as continuous and context-dependent.

==> archetypes-of-LLMs-revtex4.settings.tex <==
\newcommand{\filenamebase}{archetypes-of-LLMs}


==> archetypes-of-LLMs.author.tex <==
%% https://tex.stackexchange.com/questions/214404/add-affiliations-to-the-authors-name-in-the-article-class
%% https://tex.stackexchange.com/questions/259375/customize-author-and-affiliation-using-authblk

\renewcommand*{\Authsep}{, }
\renewcommand*{\Authand}{, }
\renewcommand*{\Authands}{, }
\renewcommand*{\Affilfont}{\normalsize\normalfont}
\renewcommand*{\Authfont}{\bfseries}
\setlength{\affilsep}{2em}


\renewcommand*{\Authsep}{, }
\renewcommand*{\Authand}{, }
\renewcommand*{\Authands}{, }
\renewcommand*{\Affilfont}{\normalsize\normalfont}
\renewcommand*{\Authfont}{\bfseries}
\setlength{\affilsep}{2em}

\author[1\thanks{shun.zhang@uvm.edu}]{Shun~Zhang}
\author[1,2]{Tabia~Tanzin~Prama}
%% tabia.prama@uvm.edu
\author[1,3]{Christopher~M.~Danforth}
\author[1,2,4,5\thanks{peter.dodds@uvm.edu}]{Peter~Sheridan~Dodds}

\affil[1]{
  Computational Story Lab,
  Vermont Complex Systems Institute,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Center,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}
\affil[2]{
  Department of Computer Science,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}
\affil[3]{
  Department of Mathematics \& Statistics,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}
\affil[4]{
  Santa Fe Institute,
  1399 Hyde Park Rd,
  Santa Fe,
  NM 87501,
  US
}
\affil[5]{
  Complexity Science Hub,
  Metternichgasse 8,
  1030 Vienna,
  Austria
}




==> archetypes-of-LLMs.biblio.tex <==
\bibliography{\filenamebase}


==> archetypes-of-LLMs.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}


==> archetypes-of-LLMs.contributions.tex <==
Who did what.


==> archetypes-of-LLMs.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> archetypes-of-LLMs.outtakes.tex <==
Long abstract:


Computational narrative analysis increasingly seeks representations that capture how language reflects changing social and interactional contexts. This study applies Ousiometry, a lexicon-based semantic framework organized around the dimensions of Power, Danger, and Structure, to the complete dialogue of the television series Friends. Using episode-level scores for the six main characters across 236 episodes, we examine temporal variation, character co-variation, and the effect of interactional context on these semantic dimensions.

Character-level trajectories show substantial episode-to-episode fluctuation. Using the PELT algorithm, we identify local change points in character trajectories, some of which align with major narrative developments. 

At the combinational level, character groups occupied different geometric positions in the Power–Danger space, with Power showing greater dispersion across group compositions than Danger. However, these positional differences do not remain statistically significant after Bonferroni correction for multiple comparisons. To evaluate the stability of episode-level measurements, split-half analyses yield generally moderate reliability across characters and dimensions, with Power showing the highest reliability overall.

Pairwise Pearson correlations further show that character trajectories exhibit nonuniform co-variation. After Bonferroni correction, only three character pairs significantly track one another across episodes in Power, two in Danger, and six in Structure. Partial correlations controlling for the remaining four main characters substantially reduce these associations. Only Monica-Chandler remains significant in power and Joey-Chandler in danger, indicating that much of the observed co-variation reflects shared ensemble-level variation. 

Overall, the results show that episode-level Ousiometry captures temporal variation in character dialogue, while evidence for stable differences among character combinations and pair-specific co-variation remains limited. They also suggest that Ousiometric variation in Friends is better characterized as continuous and context-dependent. 




% \paragraph{Change Point Interpretation}

% \todo{rewrite the interpretation for new change points}

% Several patterns emerge from the change point distribution. First, change points are not uniformly distributed across the series. Seasons 3 through 5 contain 11 of the 30 detected change points (36.7\%), a period related to the concentration of major relational transformations: the Ross-Rachel breakup, the Monica-Chandler relationship development, and the Ross-Emily marriage arc. In contrast, Seasons 6 and 10 contain the fewest change points (2 and 1), representing periods of relative stability.

% From the result, we can also detect that the change points align with specific narrative events. For example, Chandler's two Power change points at S5E09 and S5E24 precisely bracket the transition from a secret relationship to living together with Monica~\cite{wikipedia_Chandler_Bing, wikipedia_Monica_Geller}. S05E09 is just before the secret relationship with Monica being revealed, and S5E24 is when Chandler and Monica decide to live together. They both contribute to Chandler's loss of power when he is with Monica. Another piece of evidence is that Ross's three consecutive Power change points at S4E08, S5E09, and S5E14 trace the complete arc of his relationship with Emily: initiation, collapse, and acceptance. Since Ross is originally a traditionalist, a second marriage and divorce tend to be a massive turn for Ross's engagement in the ensemble's narrative~\cite{wikipedia_Ross_Geller}. The connection between PELT-detected change points and narrative events is strong and consistent. Of the 30 detected change points, 22 coincide with identifiable plot developments involving changes in various relational statuses or life transitions (The rest of the possible interpretations for all change points are in Appendix~\ref{Appendix:change_point}). These findings support the conclusion that individual sentiment arcs in Friends are closely related to narrative developments in dialogue-level Power-Danger expression.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\paragraph{ellipses}

    \begin{figure*}[ht!]
      \centering
      \includegraphics[width=0.85\linewidth]{formal_figures/confidence_ellipses.pdf}
      \caption{This figure shows the distribution of all 56 combinations on the Power-Danger plane. Each point corresponds to a unique character combination. The overall centroid of all combination means falls near $(\bar{P} = 0.0369, \bar{D} = -0.1519)$. The ellipses are the 95\% Confidence Ellipses for those character combinations. The five statistically significant deviant ones are highlighted. }
      \label{fig:confidence_ellipses}
    \end{figure*}



The ellipse areas exhibit a strong inverse relationship with scene frequency (Spearman's $\rho = -0.83$, $p < 0.001$). The six-person combination, appearing in 414 scenes, produces the smallest confidence ellipse, indicating highly precise estimation. At the opposite extreme, combinations with fewer than 15 scenes yield substantially larger ellipses. Combinations with more data support more reliable localization in the semantic space. 

We next assessed which combinations differ significantly from the global centroid. A combination is classified as significantly distinct if its 95\% confidence ellipse excludes the global centroid. By this criterion, five combinations (8.8\% of the filtered set) emerged as statistically distinct. Table~\ref{table:significant_combination} lists these combinations with their coordinates, deviation directions, and scene counts. 


\begin{table}[ht]
\centering
\small
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}Xccc>{\raggedright\arraybackslash}X}
\hline
Combination & Power & Danger & Scenes & Direction\\
\hline
Full ensemble & 0.0410 & -0.1534 & 414 & Safe Powerful\\
RcPh & 0.0420 & -0.1629 & 69 & Safe Powerful\\
PhRs & 0.0566 & -0.1483 & 38 & Danger Powerful\\
RcPhChRs & 0.0137 & -0.1530 & 12 & Safe Weak\\
RcPhJyChRs & 0.0326 & -0.1644 & 17 & Safe Weak\\
\hline
\end{tabularx}
\caption{Combinations that are significantly distinct from the global centroid. Each displays relative mean power and danger scores, scene counts and deviation direction. }
\label{table:significant_combination}
\end{table}



Based on the ellipse Figure~\ref{fig:confidence_ellipses} and Table~\ref{table:significant_combination}, we can see that no combination falls into the Low Power and High Danger quadrant, which is the Weak-Danger direction. Weak-Danger direction indicates that characters are simultaneously lacking power while facing elevated conflict or threat. This usually happens in situations including tragedy or crime drama. So the absence may reflect the show's genre: an everyday sitcom dialogue. Even in moments of conflict, the characters are more likely to engage in interactions that maintain a comedic atmosphere. 

\subsubsection{Interpretation of Deviant Combinations}
Specifically, we look into those 5 significant combinations. The six-person combination appears in more scenes than any other grouping and yields the most precisely estimated position in the space. Its location aligns with the narrative function of full-group scenes, which involve extensive decision-making, mutual support, and the resolution of ongoing storylines. 

The Rachel-Phoebe group is also towards this direction (Power-Safe). These two former roommates actually produce the second-lowest Danger score among all significant combinations. This pair's dialogue often centers on romantic counsel or everyday solidarity, which exemplifies supportive friendship. The high Power likely stems from their mutual active and solution-oriented characteristics.

Phoebe and Ross are among the most interesting pairs on the show. This pair presents the most unusual profile. Both characters individually occupy positions near the centroid, yet their joint appearance leads to the highest Power score across all combinations and a high Danger way above the ensemble average. The combination appears in only 38 scenes, suggesting that these interactions are infrequent but intense. Looking back at the show's storyline, certain interactions between Phoebe and Ross characterized by "intellectual friction" stand out in particular. For instance, Phoebe’s unconventional challenges to Ross’s scientific worldview are impressive and become the most interesting debates of the series. One of the most notable conversations is in S02E03, where she questions the theory of evolution.
\begin{quote}
\textbf{Ross:} You don't believe in evolution?\\
\textbf{Phoebe:} ...I just think it's a little too easy.\\
\textbf{Ross:} Too easy? The process of every living thing on this planet evolving over millions of years from single-celled organisms—too easy?\\
\textbf{Phoebe:} Yeah, I just don't buy it.\\
\textbf{Ross:} Evolution is not for you to buy, Phoebe. Evolution is scientific fact, like the air we breathe, like gravity.\\
\end{quote}
The ensuing dialogue combines strong displays of individual insistence on one's position with an elevated level of interpersonal conflict. 


The remaining significant combinations both exclude Monica, and they both towards Weak-Safe direction. The four-person set (Rachel + Phoebe + Chandler + Ross) exhibits the lowest Power overall, while the five-person set excluding Monica (Rachel + Phoebe + Joey + Chandler + Ross) yields the lowest Danger overall. This pattern suggests that Monica's presence systematically elevates Power in group configurations. This finding is consistent with her narrative role as the group's organizer and rule-enforcer. Traits like Neatness and hygiene are  her main labels proven by that Monica categorizes her towels into eleven separate categories (mentioned in the lightning round in S04E12)~\cite{wikipedia_Monica_Geller}. When she is absent, dialogue loses powerful force and usually occupies a more gentle and less confrontational semantic region.

The significance of these five combinations lies in the close correspondence between their Power–Danger profiles and their established narrative profiles. This coherence strengthens the claim that Power-Danger positions encode meaningful narrative and social information.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\paragraph*{Cluster Interpretation}

Figure~\ref{fig:cluster_trajectories} visualizes all six trajectory clusters in Power-Danger space.
    \begin{figure*}[ht!]
      \centering
      \includegraphics[width=0.85\linewidth]{formal_figures/all_clusters_power_danger_trajectories_2x2.pdf}
      \caption{Mean power trajectories of character-combination clusters across the ten seasons of Friends. Character combinations are clustered according to the similarity of their seasonal Power–Danger trajectories using Dynamic Time Warping (DTW) and hierarchical clustering. Each panel corresponds to one trajectory cluster, with the member character combinations listed in the upper-left corner. Thin semi-transparent lines represent the seasonal power trajectories of individual character combinations, while the bold colored line denotes the cluster mean trajectory. }
      \label{fig:cluster_trajectories}
    \end{figure*}

The DTW-based hierarchical clustering identifies four recurrent patterns of temporal evolution in the Power–Danger space. These clusters are interpreted according to the shapes of their trajectories.

Cluster 1: Power-Fluctuating. This cluster is characterized by fluctuations in Power across the series, while Danger remains comparatively stable. Power rises in the early seasons, falls around Season 3, increases substantially toward the middle of the series, declines again, and then rises toward the final seasons. Rather than following a consistent upward or downward direction, the trajectory repeatedly shifts between higher- and lower-Power states. The relative stability of Danger suggests that the distinguishing feature of this pattern is primarily variation along the Power dimension.

Cluster 2: Fluctuation-to-Stability. This cluster is characterized by a transition from larger variability in the earlier seasons to a more stable pattern in the later seasons. These trajectories exhibit relatively pronounced fluctuations during the first half of the series, particularly along the Power dimension, whereas these differences become less pronounced toward the later seasons. Danger shows a similar tendency. This cluster thus suggests a shift from relatively unstable early dynamics toward stability over the course of the series. This pattern is also broadly consistent with the narrative arcs represented by the three combinations in this cluster. Both Ross and Joey undergo substantial relational and personal changes in the earlier seasons, while their narrative roles become more established later in the series\cite{wikipedia_Ross_Geller, wikipedia_Joey_Tribbiani}. Most notably, Monica and Chandler transition from being separate in the earlier series to an established romantic relationship and eventually marriage in the end\cite{wikipedia_Monica_Geller, wikipedia_Chandler_Bing}. Their general progression from greater early instability toward more established later states parallels the fluctuation-to-stability pattern identified in their Power–Danger trajectories.

Cluster 3: Decline-and-Recovery. This cluster displays the clearest directional temporal structure. Power begins at a relatively high level, declines in the early seasons, and stabilizes in the later seasons. Danger varies to a lesser extent and does not exhibit an equivalent long-term shift. The high-power start distinguishes it from the comparatively stable trajectories of Cluster 4. 

Cluster 4: Stable. The largest cluster represents a comparatively stable temporal pattern. Both Power and Danger remain within relatively narrow ranges across the ten seasons. This pattern suggests that many character configurations maintain a relatively consistent position in the Power–Danger space over the course of the series rather than undergoing substantial long-term transformations. Notably, this cluster contains many of the larger character combinations, including the five- and six-character combinations. This compositional pattern suggests that scenes involving larger groups tend to exhibit more stable aggregate Power–Danger dynamics over time.

In all, the four clusters reveal that character configurations differ in where and how they move through power-danger space over time. The DTW analysis complements the static comparison of character configurations by identifying recurrent forms of temporal organization in their ousiometric trajectories. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{table}[ht!]
\centering
\begin{tabular}{c l}
\hline
\textbf{Cluster} & \textbf{Character Combinations}  \\
\hline
1 & Rachel; Rachel-Phoebe;  \\
2 & Joey; Monica-Chandler; Ross;  \\
3 & Monica-Phoebe; Phoebe; Phoebe-Joey;  \\
4 & Chandler; Joey-Chandler; Joey-Chandler-Ross; \\
& Rachel-Ross; Rachel-Monica-Phoebe; \\
& Rachel-Monica-Phoebe-Joey-Chandler;  \\
& Rachel-Monica-Phoebe-Joey-Chandler-Ross  \\
\hline
\end{tabular}
\caption{The result for trajectory clustering}
\label{tab:rq3_clusters}
\end{table}













